Deep Layer-wise Networks Have Closed-Form Weights

There is currently a debate within the neuroscience community over the likelihood of the brain performing backpropagation (BP). To better mimic the brain, training a network $\textit{one layer at a time}$ with only a "single forward pass" has been proposed as an alternative to bypass BP; we refer to these networks as "layer-wise" networks. We continue the work on layer-wise networks by answering two outstanding questions. First, $\textit{do they have a closed-form solution?}$ Second, $\textit{how do we know when to stop adding more layers?}$ This work proves that the kernel Mean Embedding is the closed-form weight that achieves the network global optimum while driving these networks to converge towards a highly desirable kernel for classification; we call it the $\textit{Neural Indicator Kernel}$.

==> tex/h_conclusion.tex <==
\textbf{Conclusion. }
We presented two exciting questions for the Neuroscience community and answered affirmatively for both. The evidence suggests that BP and SGD is not a prerequisite to train a highly effective network for classification. Indeed, due to the trivial computation requirement of $W_s$, this solution suggests that networks (potentially the brain) can classify any data using only a repetition of simple operations. Beyond this finding, we also demonstrated how the network limit behavior could help to identify the network depth. These patterns are predictable by our theorems and reproducible experimentally. Therefore, we hope these finding can open the door to new research relating artificial to biological neural networks.
\clearpage

==> tex/k_broader_impact.tex <==
\textbf{Broader Impact. } Finding an alternative to BP also has significant climate implications.   \citet{strubell2019energy} have shown that some standard AI models can emit over 626,000 pounds of carbon dioxide; a carbon footprint five times greater than the lifetime usage of a car. Therefore, the environmental impact of BP necessitates a cheaper alternative. Looking at nature, we can be inspired by the brain's learning capability using only a fraction of the energy. Perhaps artificial neurons can also train without the high energy cost to the environment. To mimic the brain, learning the network one layer at a time has been proposed as a more likely candidate to match existing understandings in Neuroscience \citep{ma2019hsic,Pogodin2020KernelizedIB}. This work aims to bypass BP with these layer-wise networks and answer the following two theoretical questions.

==> tex/m_checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}
%\answerYes{}, \answerNo{}, or \answerNA{}
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{} \\
    \textbf{Justification. } \textit{The central contribution of this work is presented as Theorem 1 and 2. These two findings answer the two main questions raised in the abstract/Intro. Namely, we have first shown that SGD and backpropagation are not prerequisites to training a network for classification given the closed-form solution $W_s$. We have secondarily shown the mathematical viability of learning the network depth via a network convergence behavior. Moreover, we purposely designed the experiments to test each theoretical claim carefully. Therefore, both the theorems and the experiments are structured to reinforce our contributions as proposed in abstract/Into.} 
  \item Did you describe the limitations of your work?
    \answerYes{} \\
    \textbf{Justification. }  \textit{See the last section of the last page under the title "Limitations." }
  \item Did you discuss any potential negative societal impacts of your work?
     \answerYes{} \\
    \textbf{Justification. }  \textit{Since our work is at such a fundamental and theoretical level, it would be difficult or even impossible to foresee its immediate implication. However, we felt that a key motivation of this work will have a significant societal impact and should be discussed by the community. 
    %Since the checklist will be made public, we have decided to add a small "Broader Impact" section here.
    } \\
    \begin{adjustwidth}{0.2in}{0.2in}
    \textbf{Broader Impact. } 
    Finding an alternative to BP also has significant climate implications.   \citet{strubell2019energy} have shown that some standard AI models can emit over 626,000 pounds of carbon dioxide; a carbon footprint five times greater than the lifetime usage of a car. This level of emission is simply not sustainable in light of our continual explosive growth. Therefore, the environmental impact of BP necessitates a cheaper alternative. Looking at nature, we can be inspired by the brain's learning capability using only a fraction of the energy. Perhaps artificial neurons can also train without the high energy cost to the environment. This is the moral and the foundational motivation for this work in identifying the existence of $W_s$. A closed-form solution holds the potential to significantly reduce the computational requirement and carbon footprint.  Even if our work ultimately failed to mimic the brain, we hope to inspire the community to identify other closed-form solutions and go beyond BP. \\ \\
    This paper aims to promote the discussion of viewing backpropagation alternatives not only as an academic exercise but also as a climate imperative. Yet, this topic is largely ignored by the community. The authors believe the energy costs of training Neural Networks are having a detrimental climate impact and should be an added topic of interest in NeurIPS along with fairness and racial equality. The earth also needs an advocate, why not us? Therefore, we as a community, must begin addressing how we can ameliorate our own carbon footprint. This exploratory work aims to share a potential path forward for further research that may address these concerns with the community. While $W_s$ is still not ready for commercial usage, we sincerely hope that the community begins to build novel algorithms over our work on \RS and identify a simpler and cheaper path to train our networks. \\
    \end{adjustwidth}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
      \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
      \answerYes{} \\
    \textbf{Justification. }  \textit{We have to the best of our ability state the necessary assumptions. Since the authors are not infallible, it is possible to have oversights. We would be happy to incorporate any suggestions from the reviewers. }
	\item Did you include complete proofs of all theoretical results?
    \answerYes{} \\
    \textbf{Justification. } \textit{We have proven Theorem 1 in Appendix A, and Theorem 2 in Appendix B. Corollary 1 and 2 are proven in Appendix D. For reproducibility, we have purposely written the proof to be instructional. This means that we have clearly defined each symbol and tediously wrote the proof step by step without skipping operations that may appear obvious to a more senior audience. We note that this is not intended to insult the intelligence of reviewers, but it is designed to help younger students to reproduce, understand, and build upon the proof.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{} \\
    \textbf{Justification. } \textit{The source code to implement $W_s$ and $W^*$ are included in the Supplementary materials along with simple instructions to run them. We worked to ensure that the experimental results are easily reproducible in several manners. First, repeating each experiment is as simple as uncommenting the experiment you wish to run. Second, we also included the exact data used to conduct each experiment. Third, we also included the code we used for the competing methods to allow the comparisons easily reproducible. Therefore, the entire process is public, can be examined by any individual, and yields results that should closely track the paper. }
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} \\
    \textbf{Justification. } \textit{The training detail to conduct the experiments are describe in the Experiment section under the subtitle "Evaluation Metrics" and "Experiment Settings". There are also hyperparameter choices that are less obvious, e.g., how did we choose the $\sigma$ value for the Gaussian kernel? For this, we included in App. \ref{app:opt_sigma} a detailed description for the logic behind how they were identified. We even conducted additional experiments and provided figures (also included in the appendix) to demonstrate how it works in practice. The source code for $\sigma$ identification is included with the Supplementary Material.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{} \\
    \textbf{Justification. } \textit{Every single experiment is conducted with 10-fold cross validation. This implies that each dataset is randomly divided into 10 subsets. Every experiment is conducted 10 times using each 10\% subset as the test set and the 90\% as the training. We then collect the mean and the standard deviation for each 10-fold experiment and report these values in the format $\mu \pm \sigma$.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{} \\
    \textbf{Justification. } \textit{The computation device description is included along with "Experiment Settings".}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
     \answerYes{} \\
    \textbf{Justification. } \textit{For every single data and every competing method, we cite the work immediately after mentioning the source. These citations can be found from the first two paragraphs of the Experimental section. Every dataset is also included in the Supplementary. The link to download the original dataset is also included in App.~\ref{app:data_detail}. For each competing method, the link to download the source code from github is included in the reference. These citations can be found from the first two paragraphs of the Experimental section. } 
  \item Did you mention the license of the assets?
     \answerNA{}  \\
     \textbf{Justification. } We have purposely used datasets that are in the public domain. The license information can be easily obtained from the link provided within the paper.
  \item Did you include any new assets either in the supplemental material or as a URL?
     \answerNA{} 
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
     \answerNA{} 
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
    %\textbf{Justification. } \textit{Since the datasets are already well known as standard datasets researchers use, we believe they are sufficiently innocuous to skip this question. }
  %\answerNo{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

